The minimal communication cost for simulating entangled qubits

We analyze the amount of classical communication required to reproduce the statistics of local projective measurements on a general pair of entangled qubits, $|\Psi_{AB}>=\sqrt{p}\ |00>+\sqrt{1-p}\ |11>$ (with $1/2\leq p \leq 1$). We construct a classical protocol that perfectly simulates local projective measurements on all entangled qubit pairs by communicating one classical trit. Additionally, when $\frac{2p(1-p)}{2p-1} \log{\left(\frac{p}{1-p}\right)}+2(1-p)\leq1$, approximately $0.835 \leq p \leq 1$, we present a classical protocol that requires only a single bit of communication. The latter model even allows a perfect classical simulation with an average communication cost that approaches zero in the limit where the degree of entanglement approaches zero ($p \to 1$). This proves that the communication cost for simulating weakly entangled qubit pairs is strictly smaller than for the maximally entangled one.

==> 0_MTQ_macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   Begin Macros
%Useful math and quantum information macros
\newcommand{\ket}[1]{\vert#1\rangle}
\newcommand{\dket}[1]{\vert#1\rangle\hspace{-.8mm}\rangle}
\newcommand{\dketBIG}[1]{\Big\vert#1\Big\rangle\hspace{-.8mm}\Big\rangle}
\newcommand{\bra}[1]{\langle#1\vert}
\newcommand{\dbra}[1]{\langle\hspace{-.8mm}\langle #1\vert}
\newcommand{\braket}[2]{\langle#1\vert#2\rangle}
\newcommand{\ketbra}[2]{\vert #1 \rangle \hspace{-.4mm} \langle #2 \vert}
\newcommand{\dketbra}[2]{\vert #1 \rangle \hspace{-.8mm} \rangle \hspace{-.4mm} \langle\hspace{-.8mm}\langle #2 \vert}
\newcommand{\dketbraBIG}[2]{\Big\vert #1 \Big\rangle \hspace{-.8mm} \Big\rangle \hspace{-.4mm} \Big\langle\hspace{-.8mm}\Big\langle #2 \Big\vert}
%\newcommand{\1}{\mathbb{1}}
\newcommand{\1}{\mbox{1}\hspace{-0.25em}\mbox{l}}
\newcommand{\id}{\mathds{1}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\sgn}{sgn}
\newcommand*\dif{\mathop{}\!\mathrm{d}}
\newcommand{\mean}[1]{\left\langle#1\right\rangle}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\ind}{\operatorname{ind}}
\newcommand{\abs}[1]{\left|#1\right|}
%%Useful italic macros
\newcommand{\st}{\text{s.t.}}
\newcommand{\etal}{\textit{et al}. }
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}
%Useful Spaces
\renewcommand{\H}{\mathcal{H}}
\renewcommand{\P}{\mathcal{P}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\A}{\mathcal{A}}
\renewcommand{\j}{\mathcal{j}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\C}{\mathfrak{C}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\SU}{\mathcal{SU}}
\newcommand{\im}{\mathrm{i}}
%Floor and Ceil function
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
%The double tilde from https://tex.stackexchange.com/questions/321231/double-widetilde
\makeatletter 
\newcommand{\doublewidetilde}[1]{{%
  \mathpalette\double@widetilde{#1}%
}}
\newcommand{\double@widetilde}[2]{%
  \sbox\z@{$\m@th#1\widetilde{#2}$}%
  \ht\z@=.9\ht\z@
  \widetilde{\box\z@}%
}
%Add tilde for linear maps and supermaps
\newcommand{\map}[1]{\widetilde{#1}}  
%\newcommand{\smap}[1]{\widetilde{\widetilde{#1}}}
\newcommand{\smap}[1]{\doublewidetilde{{#1}_{}}}
\newcommand{\set}[1]{\mathsf{#1}}
\makeatother
%Colour related macros
\newcommand{\MT}[1]{\textcolor{magenta}{[MT: #1]}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\pink}[1]{\textcolor{magenta}{#1}}
% Theorem enviroment
\newtheorem{conjecture}{Conjecture}
\newtheorem{result}{Main Result}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{notation}{Notation}
\newtheorem{proposition}{Proposition}
%Macros for institutions
\newcommand{\todai}{Department of Physics, Graduate School of Science, The University of Tokyo, Hongo 7-3-1, Bunkyo-ku, Tokyo 113-0033, Japan}
\newcommand{\univie}{Faculty of Physics, University of Vienna, Boltzmanngasse 5, 1090 Vienna, Austria}
\newcommand{\IQOQI}{Institute for Quantum Optics and Quantum Information (IQOQI), Austrian Academy of Sciences, Boltzmanngasse 3, A-1090 Vienna, Austria}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   End Macros
